Fixed-Confidence Guarantees for Bayesian Best-Arm Identification

We investigate and provide new insights on the sampling rule called Top-Two Thompson Sampling (TTTS). In particular, we justify its use for fixed-confidence best-arm identification. We further propose a variant of TTTS called Top-Two Transportation Cost (T3C), which disposes of the computational burden of TTTS. As our main contribution, we provide the first sample complexity analysis of TTTS and T3C when coupled with a very natural Bayesian stopping rule, for bandits with Gaussian rewards, solving one of the open questions raised by Russo (2016). We also provide new posterior convergence results for TTTS under two models that are commonly used in practice: bandits with Gaussian and Bernoulli rewards and conjugate priors.

==> appendices/app_future.tex <==
\section{Future work}\label{app:future}

% In this paper, we provided a fixed-confidence analysis for \TTTS. It would also be meaningful to provide a fixed-budget analysis, in particular in some potential application scenario of \TTTS. For example, pure exploration bandit algorithms are widely used in \emph{hyper-parameter optimization} for machine learning~\citep{hoffman2014bayesgap,li2017hyperband,shang2019dttts}.
% 
% 
% Another important unsolved open question comes to the tuning of $\beta$. Indeed, if $\beta$ is set to $\beta^\star = \argmax_{\beta \in [0,1]} \Gamma_\beta^\star$, a $\beta$-optimal strategy is also optimal. In practice of course $\beta^\star$ is unknown and so far \TTTS cannot be asymptotically optimal without this knowledge. However, note that \cite{russo2016ttts} shows that $\Gamma^\star_{1/2} \geq \Gamma^{\star}/2$, which provides a near-optimal tuning of \TTTS. Obviously, proposing an satisfying online tuning of $\beta$ (other than the one proposed in the \TTTS paper) with provable fixed confidence guarantees is another avenue for future work.
% 
% There is another line of research that leverages a game theoretic point of view on the pure exploration setting, that explores a statistic-computation trade-off~\citep{menard2019lma,degenne2019solvinggame}. One open question is to investigate whether Thompson Sampling-based exploration can replace the current (complicated) optimistic approach.

% Finally, it is also interesting to know whether there exist better sampling methods, that can accelerate the procedure of sampling the challenger.


==> appendices/app_optimal_weight.tex <==
\section{Existence and uniqueness of the optimal proportion vector}\label{app:optimal_weight}

\restateoptim*

\begin{proof}
We handle the existence and the uniqueness separately as below.
    ~\paragraph{Existence} For any arm $i\neq I^\star$, $C_i$ is a continuous function, so as to $\min_{i\neq I^\star} C_i$. According to the \emph{extreme value theorem}, function $\min_{i\neq I^\star} C_i(\beta,\cdot)$ must attain its maximum over $[0,1]^{K-1}$ which is compact. Suppose that $\bomega^\beta$ is a such maximizer. We thus have
    \[
        \Gamma_{\beta}^\star = \max_{\bomega:\omega_{I^\star}=\beta}\min_{i\neq I^\star} C_i(\beta,\omega_i) = \min_{i\neq I^\star} C_i(\beta,\omega_i^\beta).
    \]
    Let us assume that $\bomega^\beta$ does not verify the second condition, which means there exists some $j\neq I^\star$ such that
    \[
        C_j(\beta,\omega_i^\beta) > C_{i^\star}(\beta,\omega_{i^\star}^\beta),
    \]
    where $i^\star \eqdef \argmin_{i\neq I^\star} C_i(\beta,\omega_i^\beta)$.
    Now if we subtract a small quantity $\epsilon>0$, from $C_j(\beta,\omega_j^\beta)$, such that
    \[
    \epsilon \leq \frac{C_j(\beta,\omega_j^\beta)-C_{i^\star}(\beta,\omega_{i^\star}^\beta)}{2},
    \]
    and add $\epsilon/(K-2)$ to $C_i(\beta,\omega_i^\beta)$ for any $i\neq j,I^\star$, we would not change the order of the $C_i(\beta,\omega_i^\beta)$. Therefore, $i^\star$ remains unchanged, however, the new $C_{i^\star}(\beta,\omega_{i^\star}^\beta)$ would be strictly larger than the previous one which contradicts the definition of $\bomega^\beta$.

    ~\paragraph{Uniqueness} We now need to show that the solution is unique. Suppose that two different maximizers $\bomega$ and $\bomega'$ exist, and there exists some $i\neq I^\star$ such that $\omega_i > \omega'_i$. Since $C_i(\beta,\cdot)$ is an strictly increasing function, thus we have $C_i(\beta,\omega_i)>C_i(\beta,\omega'_i)$. By consequence, for any $j\neq i$ and $j'\neq i$,
    \[
        C_j(\beta,\omega_j) = C_i(\beta,\omega_i) > C_i(\beta,\omega'_i) = C_{j'}(\beta,\omega'_{j'}).
    \]
    Therefore, for any $j\neq I^\star$ and $j'\neq I^\star$, $\omega_j > \omega'_j$, and
    \[
        \sum_{j\neq I^\star} \omega_j > \sum_{j\neq I^\star} \omega'_j.
    \]
    However, we know that $1-\sum_{j\neq I^\star} \omega_j = \omega_{I^\star} =  \beta = \omega'_{I^\star} = 1-\sum_{j\neq I^\star} \omega'_j$, contradiction!
\end{proof}


==> appendices/app_pac_gaussian.tex <==
\section{Proof of \texorpdfstring{$\delta$-}{}correctness}\label{app:pac_gaussian}

We hereby demonstrate Theorem~\ref{thm:pac_gaussian}. 

\restatepac*

For that purpose, we need the Gaussian tail inequality of Lemma~\ref{lemma:gaussiantails}. Now recall that what we want to show is that for a given $\delta\in (0,1)$,
\begin{equation*}
    \underbrace{\PP{\tau_{\delta} < \infty, J_{\tau_{\delta}}^{(1)} \neq I^\star}}_\text{(*)} \leq \delta
\end{equation*}
for a certain threshold $c_{n,\delta}$ to be determined.

\begin{proof}
Using the union bound, we have
\begin{align*}
\begin{split}
    \text{(*)} &= \PP{\bigcup_{i\neq I^\star} \left\{ \tau_{\delta} < \infty, J_{\tau_{\delta}}^{(1)} = i \right\}} \\
                  &\leq \sum_{i\neq I^\star} \PP{\tau_{\delta} < \infty, J_{\tau_{\delta}}^{(1)} = i} \\
                  &= \sum_{i\neq I^\star} \PP{\exists t \in \NN, a_{t,i} \geq c_{t,\delta}}.
\end{split}
\end{align*}

%We can be more precise on $a_{n,i}$. As we already stated in the main text, under improper priors with $\mu_{1,i}=0$ and $\sigma_{1,i}=+\infty$ for any $i\in\cA$, it is easy to compute the true posterior mean (which is identical to the empirical mean) and the posterior variance,
%\[
%    \mu_{n,i} = \hat{\mu}_{n,i} = \frac{1}{T_{n,i}} \sum_{l=1}^{n-1} \1\{I_l = i\}Y_{l,I_l}, \sigma_{n,i}^2 = \frac{\sigma^2}{T_{n,i}},
%\]
%and the posterior distribution can be written as
%\[
%    \Pi_{n} = \bigotimes_{i=1}^{K} \cN\left( \mu_{n,i}, \frac{\sigma^2}{T_{n,i}} \right).
%\]

%Therefore $\forall i\in\cA$ and $n\in\NN$,
%\begin{align*}
%\begin{split}
%    a_{n,i} &= \mathbb{P}_{\btheta\sim\Theta}\left[\theta_i > \max_{j\neq i} \theta_j \right] \\
%                 &= \int_{\Theta_i} \prod_{i=1}^{K} \frac{1}{\sqrt{2\pi}\sigma^2/T_{n,i}} \expp{-\frac{(\theta_i-\mu_{n,i})^2}{2\sigma^2/T_{n,i}}} d\btheta \\
%                 &= \int_{\Theta_i} \frac{1}{(\sqrt{2\pi}\sigma^2/T_{n,i})^K} \expp{-\sum_{i=1}^K\frac{(\theta_i-\mu_{n,i})^2}{2\sigma^2/T_{n,i}}} d\btheta. \\
%\end{split}
%\end{align*}

%The previous form is closely related to that of Conjecture Lemma~\ref{lemma:posterior}, since in the Gaussian case, $d(\mu_i;\theta_i) = \frac{(\theta_i-\mu_i)^2}{2\sigma^2}$.

At the end of round $n$, the algorithm would choose a wrong arm if there exists $i\neq I^\star$, s.t.
\[
	a_{n,i} \geq c_{n,\delta},
\]
which implies in particular,
\begin{equation}\label{eq:error}
	\Pi_{n}\left[\theta_i \geq \theta_{I^\star} \right] \geq c_{n,\delta}.
\end{equation}

The threshold $c_{n,\delta}$ is a large number ($>1/2$), thus the wrong pick could only occur if the posterior mean of arm $i$ is larger than the posterior mean of the true best arm $I^\star$,
\[
    \mu_{n,i} \geq \mu_{n,I^\star}.
\]
We are then prepared to apply Lemma~\ref{lemma:gaussiantails}. Since we have
\begin{align*}
    (\ref{eq:error}) &\iff 1 - \Pi_{n}\left[\theta_i < \theta_{I^\star} \right] \geq c_{n,\delta} \\
                     &\iff 1 - c_{n,\delta} \geq \Pi_{n}\left[\theta_i - \theta_{I^\star} < 0 \right] \\
\end{align*}
and rewriting $\Pi_{n}\left[\theta_i - \theta_{I^\star} < 0 \right]$ as 
\[
\Pi_{n}\left[\theta_i - \theta_{I^\star} < \mu_{n,i} - \mu_{n,I^\star} + \mu_{n,I^\star} - \mu_{n,i} \right],
\]
then applying Lemma~\ref{lemma:gaussiantails} with $c = \mu_{n,I^\star} - \mu_{n,i} \leq 0$, we obtain
\begin{align*}
    1 - c_{n,\delta} &\geq \frac{1}{\sqrt{2\pi}} \expp{-\frac{1}{2\sigma_{n,i,I^\star}^2}\left( \sigma_{n,i,I^\star}+\mu_{n,i}-\mu_{n,I^\star} \right)^2},
\end{align*}
where $\sigma_{n,i,I^\star} \eqdef \sqrt{\sigma^2/T_{n,i}+\sigma^2/T_{n,I^\star}}$. Hence, we have
\[
    \ln{\frac{1}{\sqrt{2\pi}(1-c_{n,\delta})}} \leq \frac{1}{2\sigma_{n,i,I^\star}^2}\left( \sigma_{n,i,I^\star}+\mu_{n,i}-\mu_{n,I^\star} \right)^2.
\]
We take square root of both sides since we know how to control $(\mu_{n,i}-\mu_{n,I^\star})^2/(2\sigma_{n,i,I^\star}^2)$, 
\[
    \sqrt{\ln{\frac{1}{\sqrt{2\pi}(1-c_{n,\delta})}}} - \frac{1}{\sqrt{2}} \leq \frac{1}{\sqrt{2}\sigma_{n,i,I^\star}} (\mu_{n,i}-\mu_{n,I^\star}),
\]
and finally,
\[
    \left( \sqrt{\ln{\frac{1}{\sqrt{2\pi}(1-c_{n,\delta})}}} - \frac{1}{\sqrt{2}} \right)^2 \leq \frac{(\mu_{n,i}-\mu_{n,I^\star})^2}{2\sigma_{n,i,I^\star}^2},
\]

Now we need to bound $(\mu_{n,i}-\mu_{n,I^\star})^2/(2\sigma_{n,i,I^\star}^2)$. We know that
\begin{align*}
    \frac{(\mu_{n,i}-\mu_{n,I^\star})^2}{2\sigma_{n,i,I^\star}^2} &= \inf_{\theta_i<\theta_{I^\star}} T_{n,i}d(\mu_{n,i};\theta_i) + T_{n,I^\star}d(\mu_{n,I^\star};\theta_{I^\star}),
\end{align*}
and using a result in Theorem 10 of~\citet{garivier2016tracknstop}, we know that if $\mu_{n,i} \geq \mu_{n,I^\star}$, then for any $\delta>0$,
\[
    \PP{\exists n\in\NN, \frac{(\mu_{n,i}-\mu_{n,I^\star})^2}{2\sigma_{n,i,I^\star}^2} > \ln{\frac{2n(K-1)}{\delta}}} \leq \frac{\delta}{K-1}.
\]
Note that the statistic $Z_n$ used by~\citet{garivier2016tracknstop} is exactly equal to $\inf_{\theta_i<\theta_{I^\star}} T_{n,i}d(\mu_{n,i};\theta_i) + T_{n,I^\star}d(\mu_{n,I^\star};\theta_{I^\star})$ in our Gaussian case.

Now denoting $\kappa_{n,\delta} \eqdef \left( \sqrt{\ln(1/(\sqrt{2\pi}(1-c_{n,\delta})))} - 1/\sqrt{2} \right)^2$, it suffices to set $\kappa_{n,\delta}$ to be equal to $\ln{2n(K-1)/\delta}$ so that for any $\delta > 0$,
\begin{align*}
\begin{split}
    \text{(*)} &\leq \sum_{i\neq I^\star} \PP{\exists t \in \NN, a_{t,i} \geq c_{t,\delta}} \\
    &\leq \sum_{i\neq I^\star} \PP{\exists t \in \NN, \frac{(\mu_{t,i}-\mu_{t,I^\star})^2}{2\sigma_{t,i,I^\star}^2} \geq \kappa_{t,\delta}} \\
    &\leq (K-1)\max_{i\neq I^\star} \PP{\exists t \in \NN, \frac{(\mu_{t,i}-\mu_{t,I^\star})^2}{2\sigma_{t,i,I^\star}^2} \geq \kappa_{t,\delta}} \\
    &\leq \delta.
\end{split}
\end{align*}
\end{proof}

By a simple computation, it suffices to set the threshold as
\[
    c_{n,\delta} \eqdef 1 - \ddfrac{\delta}{2n(K-1)\sqrt{2\pi e}\expp{\sqrt{2\ln{\frac{2n(K-1)}{\delta}}}}}
\]
to make sure that for any $\delta > 0$, $\PP{\tau_{\delta} < \infty, J_{\tau_{\delta}}^{(1)} \neq I^\star} \leq \delta$.

The previous result can be further refined since $\inf_{\theta_i<\theta_{I^\star}} T_{n,i}d(\mu_{n,i};\theta_i) + T_{n,I^\star}d(\mu_{n,I^\star};\theta_{I^\star})$ can be precisely bounded by $T_{n,i}d(\mu_{n,i};\mu_i) + T_{n,I^\star}d(\mu_{n,I^\star};\mu_{I^\star})$. (Apply for example Corollary 10 by~\citealt{kaufmann2018mixture}.)


==> appendices/app_rate.tex <==
\section{Computation of the optimal error decay rate}\label{app:rate}

In this section, we first describe how to approximate $\Gamma_{\beta}^\star$ under any prior of 1-dimensional exponential family. We then also provide a way to compute numerically $\Gamma_{\beta}^\star$ under Gaussian prior since it can be computed more explicitly.

\subsection{General case}

For any $i\neq I^\star$, $C_i(\beta,\omega_i)$ is defined as the output to a convex minimization problem for whom the unique solution has an analytic expression
\[
    \frac{\beta}{\beta+\omega_i}\mu_{I^\star} + \frac{\omega_i}{\beta+\omega_i}\mu_i.
\]
Next, we define for any $i\neq I^\star$, a function
\begin{align*}
  g_i \colon [0,+\infty[ &\to [0,+\infty[\\
  x &\mapsto \beta d\left(\mu_{I^\star};\frac{\beta}{\beta+\omega_i}\mu_{I^\star} + \frac{\omega_i}{\beta+\omega_i}\mu_i\right) + x d\left(\mu_i;\frac{\beta}{\beta+\omega_i}\mu_{I^\star} + \frac{\omega_i}{\beta+\omega_i}\mu_i\right).
\end{align*}
In fact, $g_i$ is a strictly increasing function (see~\citealt{garivier2016tracknstop}, Appendix A.2 for more details), so does its inverse function $x_i \eqdef g_i^{-1}$ which is defined on $[0, \beta d(\mu_{I^\star};\mu_i)[$ as $g_i$ tends to 0 when $x$ tends to 0 and tends to $\beta d(\mu_{I^\star};\mu_i)$ when $x$ tends to $+\infty$.

According to Proposition~\ref{prop:optim}, the optimal proportion vector $\bomega^\beta$ that we are searching for satisfies the constraint that $\forall i,j\neq I^\star$,
\[
    g_i(\omega_i^\beta) = g_j(\omega_j^\beta) = \Gamma_{\beta}^\star.
\]
Since $\omega_i^\beta = g_i^{-1}(\Gamma_{\beta}^\star) = x_i(\Gamma_{\beta}^\star)$, and we know that $\sum_{i\neq I^\star} \omega_i = 1-\beta$, thus the problem of computing $\Gamma_{\beta}^\star$ is equivalent to solve the following equation,
\[
    \sum_{i\neq I^\star} x_i(y) = 1 - \beta.
\]
This equation has a unique solution since $\sum_{i\neq I^\star}$ is a strictly increasing function valued in $[0, +\infty[$. We can thus apply a bisection method to this function whose evaluation require itself a bisection method applied on $K-1$ smooth scalar functions.

\subsection{Gaussian case}

In the context of this paper, we can do a more efficient approximation. In the Gaussian case, we know that for any $i,j\neq I^\star$,
\[
    \frac{1}{\omega_j^\beta} + \frac{1}{\beta} = \frac{(\mu_{I^\star}-\mu_j)^2}{(\mu_{I^\star}-\mu_i)^2}\left(\frac{1}{\omega_i^\beta} + \frac{1}{\beta}\right).
\]
Denote $x_i\eqdef 1/\omega_i^\beta+1/\beta$ and $a_{ji}\eqdef (\mu_{I^\star}-\mu_j)^2/(\mu_{I^\star}-\mu_i)^2$, fix some $i\neq I^\star$, then we have $\forall j\neq I^\star$, $x_j = a_{ji}x_i$. Since $\sum_{j\neq I^\star} \omega_j^\beta = 1-\beta$, we have
\[
    \sum_{j\neq I^\star} \frac{1}{x_j-1/\beta} = \sum_{j\neq I^\star} \frac{1}{a_{ji}x_i-1/\beta} = 1-\beta.
\]
Thus we only need to find the unique solution to the equation
\[
    \sum_{j\neq I^\star} \frac{a_{ij}}{x-a_{ij}/\beta} = 1-\beta,
\]
that requires only one shot bisection method.

